Expediting DECam Multimessenger Counterpart Searches with Convolutional Neural Networks

Searches for counterparts to multimessenger events with optical imagers use difference imaging to detect new transient sources. However, even with existing artifact detection algorithms, this process simultaneously returns several classes of false positives: false detections from poor quality image subtractions, false detections from low signal-to-noise images, and detections of pre-existing variable sources. Currently, human visual inspection to remove the false positives is a central part of multimessenger follow-up observations, but when next generation gravitational wave and neutrino detectors come online and increase the rate of multimessenger events, the visual inspection process will be prohibitively expensive. We approach this problem with two convolutional neural networks operating on the difference imaging outputs. The first network focuses on removing false detections and demonstrates an accuracy of 92 percent on our dataset. The second network focuses on sorting all real detections by the probability of being a transient source within a host galaxy and distinguishes between various classes of images that previously required additional human inspection. We find the number of images requiring human inspection will decrease by a factor of 1.5 using our approach alone and a factor of 3.6 using our approach in combination with existing algorithms, facilitating rapid multimessenger counterpart identification by the astronomical community.

==> tips.tex <==
\bigskip
{\bf Some helpful tips: }

\smallskip

Remind yourself to cite something like this: \citeme{autoscan}

\smallskip

Remind yourself to check a number like this: \num{100ish}

\smallskip

Use your initials to write a note \AS{note}. \RM{note}
